Explanations for Occluded Images

Existing algorithms for explaining the output of image classifiers perform poorly on inputs where the object of interest is partially occluded. We present a novel, black-box algorithm for computing explanations that uses a principled approach based on causal theory. We have implemented the method in the DEEPCOVER tool. We obtain explanations that are much more accurate than those generated by the existing explanation tools on images with occlusions and observe a level of performance comparable to the state of the art when explaining images without occlusions.

==> background.tex <==
%\section{Background}

%\input{dnn}

\input{cause}

==> dnn.tex <==
\subsection{Deep neural networks (DNNs)}
\label{sec:dnns}

%We briefly review the relevant definitions of deep neural networks. 
Let $f: \mathcal{I} \rightarrow \mathcal{O}$ be a deep neural network $\network$ with $n$~layers. 
For a given input image $x\in \mathcal{I}$, 
$f(x)\in\mathcal{O}$ calculates the output label of the DNN. % which could be, for instance, a classification label. Images are among the most popular inputs for DNNs, and in this paper we focus on DNNs that classify images.  Specifically, we have
%
\begin{equation}\label{eq:dnn}
f(x) = f_N(\ldots f_2(f_1(x;W_1,b_1);W_2,b_2)\ldots ;W_n,b_n)
\end{equation}
%
where $W_i$ and $b_i$ for $i = 1,2,\ldots$ are learnable parameters, and $f_i(z_{i-1};W_{i-1},b_{i-1})$
is the layer function that maps the output of layer $(i-1)$, i.e., $z_{i-1}$, to the input of layer~$i$. 
%The combination of the layer functions yields highly complex behavior, and the analysis of the
%information flow within a DNN is challenging. There is a variety of layer functions for DNNs,
%including fully connected layers, convolutional layers and max-pooling layers.
%
Our algorithm is independent of the specific internals of the DNN and treats a given DNN as a black box.

==> response.tex <==

\newcommand{\marginX}{\marginnote{\huge{\quad\quad\textbf{!}\quad\quad}}}
\newcommand{\ys}[1]{{\color{blue}\marginX{}[\textbf{Youcheng}: #1]}}

\newcounter{point}
\setcounter{point}{0}

\newcommand{\var}{\textsf{Var}}

\newenvironment{revPoint}{
  \stepcounter{point}

  \hrule \medskip

  \noindent \textbf{\thepoint} Reviewer's comment: %\itshape
}
{
  \medskip
}

\newenvironment{reply}{\noindent \textbf{Reply}:\ }
{
  \\ \medskip
}    

\clearpage

\section*{Revision Letter}
\subsection*{Primary Changes}

We thank all reviewers for their kind comments and detailed suggestions. In the revision, we have highlighted all our changes. To address the reviews, we have added the results of two experiments.
%
\begin{enumerate}
    \item In Section~\ref{sec:app}, we show that our coverage-guided DNN testing can be applied to compare two different DNNs. The experiment shows that our metrics are able to drive the generation of test that quantify the robustness of the neural network very well. We also use this experiment to illustrate how a feature can be defined using the basic convolutional operation. 

    \item In Section~\ref{sec:proxy2}, we use data variety as a proxy for functional coverage. The experiment shows that the existing metrics do not approximate functional coverage at all, whereas our our metrics are very well aligned with functional coverage. This complements the other experiments in this paper that use adversarial examples as the proxy. 

\end{enumerate}

\subsection*{Reviewer \#1}
\begin{revPoint}
\begin{quote}\small\it
    bla bla
\end{quote}

\end{revPoint}


\subsection*{Reviewer \#2}

\begin{revPoint}
\begin{quote}\small\it
    bla bla
\end{quote}{}
 
\end{revPoint}{}


\subsection*{Reviewer \#3}

\begin{revPoint}
\begin{quote}\small\it
bla bla
\end{quote}

\end{revPoint}


